Backplay: "Man muss immer umkehren"

Model-free reinforcement learning (RL) requires a large number of trials to learn a good policy, especially in environments with sparse rewards. We explore a method to improve the sample efficiency when we have access to demonstrations. Our approach, Backplay, uses a single demonstration to construct a curriculum for a given task. Rather than starting each training episode in the environment's fixed initial state, we start the agent near the end of the demonstration and move the starting point backwards during the course of training until we reach the initial state. Our contributions are that we analytically characterize the types of environments where Backplay can improve training speed, demonstrate the effectiveness of Backplay both in large grid worlds and a complex four player zero-sum game (Pommerman), and show that Backplay compares favorably to other competitive methods known to improve sample efficiency. This includes reward shaping, behavioral cloning, and reverse curriculum generation.

==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}

We have trained a large number of models through our research into Backplay. Consequently, we have some empirical observations that may help with further experiments:

\begin{itemize}
    \item \textbf{Backplay performs well even when the model is trained longer on any given window.} There isn't any downside to having the model continue training in a window for too long, albeit the ideal is that this method increases the speed of training.
    \item \textbf{Backplay does not perform well when the curriculum is advanced too quickly.} In this case, it can collapse to be more like a Standard model. A scenario common to effective training is improving success curves punctured by step drops whenever the window advances that then swiftly recover.
    \item \textbf{Backplay can still recover if success goes to zero.} This surprising result frequently occurred at the juncture where the window moved back to the initial state and even if the policy's entropy over actions became maximal. We are unsure what differentiates these models from the ones that did not recover.
    \item \textbf{Backplay does not need to hit a high success rate before advancing.} Initially, we tried using adaptive approaches that advanced the window when the agent reached a certain threshold of success. This worked but was too slow. The important part is that the agent gets sufficiently exposed to enough states to attain a reasonable barometer of their value. This will then expedite later training when the window advances.
\end{itemize}

One aspect that we have considered during this research is combining Backplay with Monte Carlo Tree Search (MCTS), the algorithm largely responsible for AlphaGo and a litany of strong agents in the General Game Playing competition. These two approaches are complementary with one idea being to use Backplay as a reliable way to warm-start MCTS. We think that work in similar directions is promising.

Other future priorities are to gain a better understanding of why this works so well, where it fails, and how we can make it more efficient. Do the gains come from value estimation like our analysis suggests, from policy iteration, or from both? What about the curricula itself - is there an ideal rate at which we advance the window and is there a better approach than a hand-tuned schedule? Should we be using one policy that learns throughout training or would it be better to have a policy per window? This has some nice consequences and, if we could ascertain a confidence estimate of a state's value, will likely speed up the rate at which we can advance Backplay.

A final direction that we think is worthwhile is utilizing Backplay without generating replays beforehand. Could we develop a way for the agent to bootstrap a reasonable trajectory to use for itself? This is very difficult because the core issue is that the agent could spend an exceptionally long time achieving nothing of note in sparse environments. And, even if we could do this, how would the agent know what is reasonable when that is such a qualitative descriptor?

Last, we would like to recognize one other direction that we had planned to engage but was released simultaneously with our own work. \cite{salimans2018blog} shows that an approach very similar to Backplay can work with human demonstrations to do exceptionally well on challenging sparse environments such as Montezuma's Revenge. We think that this direction is very interesting and could lead to strong results for human in the loop training.



\subsubsection*{Acknowledgments}
We especially thank Yichen Gong, Henry Zhou, and Luvneesh Mugrai for letting us use their agent. We also thank Martin Arjovsky, Adam Bouhenguel, Tim Chklovski, Jakob Foerster, Ilya Kostrikov, and Will Whitney for helpful contributions.
